Enabling Compute-Communication Overlap in Distributed Deep Learning Training Platforms

Deep Learning (DL) training platforms are built by interconnecting multiple DL accelerators (e.g., GPU/TPU) via fast, customized interconnects with 100s of gigabytes (GBs) of bandwidth. However, as we identify in this work, driving this bandwidth is quite challenging. This is because there is a pernicious balance between using the accelerator's compute and memory for both DL computations and communication. This work makes two key contributions. First, via real system measurements and detailed modeling, we provide an understanding of compute and memory bandwidth demands for DL compute and comms. Second, we propose a novel DL collective communication accelerator called Accelerator Collectives Engine (ACE) that sits alongside the compute and networking engines at the accelerator endpoint. ACE frees up the endpoint's compute and memory resources for DL compute, which in turn reduces the required memory BW by 3.5X on average to drive the same network BW compared to state-of-the-art baselines. For modern DL workloads and different network sizes, ACE, on average, increases the effective network bandwidth utilization by 1.44X (up to 2.67X), resulting in an average of 1.41X (up to 1.51X), 1.12X (up to 1.17X), and 1.13X (up to 1.19X) speedup in iteration time for ResNet-50, GNMT and DLRM when compared to the best baseline configuration, respectively.

==> include/author_list2.tex <==
\numberofauthors{1}
\author{
  \alignauthor 
    Saaed Rashidi$^*$, Srinivas Sridharan$^\mathsection$, Sudarshan Srinivasan$^\dagger$ , Matthew Denton$^*$ and Tushar Krishna$^*$ \\                       % names
    \affaddr{$^*$Georgia Institute of Technology, Atlanta, USA }\\
    \affaddr{$^\mathsection$Facebook, Menlo Park, USA }\\            %
    \affaddr{$^\dagger$Intel, Bangalore, India }\\
    \email{saeed.rashidi@gatech.edu, ssrinivas@fb.com, sudarshan.srinivasan@intel.com}, \email{matthewdenton@gatech.edu, tushar@ece.gatech.edu}  % emails
}

==> sections/TODO.tex <==
\section{TODO}
\TODO{
\begin{itemize}
    \item Assuming alltoall sizes will be small and hence we make some design choice based on that is wrong... we cannot make the assumption alltoall size will be small. Instead say our alltoall support is tuned for small message and we will explore things in future for larger alltoall
    \item Let's avoid confusion by calling all-to-all topology ... switch topology. alltoall topology and alltoall collective is creating too much confusion
    \item Should we say "ACE" or "the ACE"? 
    \item Ensure main results takeaways are clear
    \item Spellcheck
\end{itemize}
}


==> sections/design-orig.tex <==
\section{Neural Collective Unit (NCU) Design}\label{sec:design}

\TK{I will make a detailed pass}

%% SS comments (does the following flow make sense?)
% Assume the following are already covered:
% - Hierarchical topology, algorithm mapping, SW optimization, conflicting requirements etc. 
% - Motivation for messaging agent i.e. memory contention etc. 
% - This section should focus on the following
% -- Requirements for dedicated comms agent 
% -- Design/implementation details and how the design addresses the requirements
% -- Other important topics: Transport layer / Software interface / programming model etc
% -- Ask some tough questions: what if something changes? Does HW implementation limit flexibility? 
% - We should try to introduce the term "disaggregating communication from compute" basically making the point we should be able to grow compute and comms separately. 


Altough the previous section aim was to address the growing communication size problem by carefully choosing the topology/algorithm pair, there is still a great potential in designing a hardware agent to offload the  collective communication task to it and release the NPU cores from this secondary task that is the inevitable result of the distributed training. In general, oflloading the collectives can: 1-release the valuable computation power of NPUs from performing the collective algorithms, 2-reduce the memory contention since there is no need for data to be transferred to the main memory for collective related processing. This allows the NPU cores to invest their full potential on their primary task; the training algorithm itself.

\subsection{The Overall Design}
In order to design an efficient and low-overhead messaging agent to be a good fit for the scale-up network, one needs to leverage all topology/algorithm features of the target system. This is especially important for the scale-up network because adding general-purpose components and protocols could cause significant overhead or slows down the performance, making it a bottleneck in performing collective operations. In our proposed architecture design, we leveraged the following features of the target systems (i.e. hierarchical and all-to-all topologies) to design an efficient yet simple hardware logic for the offloading task: \sri{Suggest we remove bullet points - taking too much space}
\begin{itemize}
    \item The targeted collectives, except all-to-all, have in-order access to data. On the other hand, all-to-all collectives are: 1- specific to only certain DNNs, and 2-their communication size is small compared to other collectives. This allows to simplify most of the storage elements used in the messaging agent.    
    \item The execution units can be efficiently shared among the data at different phases of the algorithm. This is because even for the phases that need local reduction (e.g. all-reduce), not all received data needs to be locally reduced (e.g. the second part of all-reduce that is all-gather), hence, the available execution resources can be shared to other phases that need local reduction. 
    \item The pipelined and multi-phase nature of target collectives running on top of hierarchical and all-to-all topologies allows to simplify and distribute the control logic of the messaging agent. This way, the control logic corresponding to each incoming link could be totally isolated from other link controllers since it only needs to know: 1-where to read data from, 2-what operation it needs to perform, and 3-where to direct/store data. 
\end{itemize}
Figure \ref{fig:MessagingAgent} shows the proposed architecture for the messaging agent with the main components labeled. It consists of several storage elements (several FIFOs and a few small sized Random Access Memories (RAMs) ) and several execution units, all connected together using multiple switches and managed by a centralized control unit (although, the control unit is divided into sub-modules). Here are the major points regarding this design: \sri{Suggest we remove bullet points - taking too much space}
\begin{itemize}
    \item The FIFOs in (\#1,\#2,\#3,\#4,\7,\#8) and RAMs (\#2) and their respective incoming/outgoing links are \textbf{logical} entities. These entities are the view of control unit from the actual storage component. This means that in reality, these storage elements might be implemented using a single SRAM bank or all of their logical input/output links might share single physical input/output link (discussed later). However, this view of observing the storage elements greatly simplifies the control unit logic while provides just enough flexibility to implement the target operations.    
    \item The control unit divides the available storage elements (i.e. FIFOs and RAMs) into logical partitions that serve as a source of data for one/multiple phases of collective communications (discussed in detail later). 
    \item The execution units (EUs) (\#5), can read from storage element as well as data coming from incoming links through switches (\#12) and (\#11). Each EU has an internal accumulate register to accumulate the results of several operations if needed (e.g. in all-to-all topologies). The output of EUs can be directed to the storage elements through backward links (\#14) and together with the incoming data can be written back to the storage elements through switch (\#13). 
    \item The unit of data processing is packet, since the packets are the units of data sent or received by the network. The bus width and FIFO slots might or might not be equal to the size of the packets and data movement/execution is serialized if the size is smaller than packet width. Also, the design does not inherently restricts the size of intra-package and inter-package packets to be the equal size.
    \item In the case of FIFOs except network FIFOs (\#8,\#9), if $P$ is the size of smallest packet in bytes, and the $F$ is the FIFO slot size, then $F>P$ and The FIFO read/write ports must be $P-byte$ addressable. This indicates that the tail and head FIFO slots provide random push and pop access to the packets residing in that slot, respectively. The FIFO write goes to the next slot once all packet rooms of the tail slot is already filled. The bus coming into/out of FIFO however, can be any size.
    \item The RAM components support all-to-all collectives because random access to data is a part of the proposed algorithms for this collective. The RAMs serve as the source for all phases of the all-to-all collective. However, RAMs can be reused as FIFOs when the workload does not require any all-to-all collective.
    \item The FIFO (\#1) and RAM (\#2) groups are the source of data movements from memory to the messaging agent and hence, they always serve as the source of first phase of collectives. There might be multiple intermediate FIFO groups (\#3 and \#4) for intermediate phases of the collective algorithm. The logical partition serving as the source for the last phase of algortihm (\#8 or \#2 for all-to-all collective) have access to the RX DMA buffer (\#7) through switch (\#6) in order to direct the final result to the main memory. Also, the switch (\#6) facilitates the express path to the output ports in order to boost the forwarding of data to output ports (e.g. useful in all-gather) and better utilize available resources by not occupying the EUs for just forwarding. Note that the storage elements with access to switch (\#6) can be placed into other partitions. However, all of the storage elements of the last step should have access to switch (\#6). 
    \item There are links (\#10), called direct links, coming out of the switch (\#13) and going to switch (\#6). They enable sending out data to the main memory directly from input ports or EU outputs. They are usefull especially for the last phase of target algorithms (discussed later in detail).
\end{itemize}
\insertFigureNew{MessagingAgent}{An overview of the proposed messaging agent}{1}
Table \ref{tab:garnularity} shows the granularity of data at different levels of the messaging agent execution and their determinative factor. The messaging agent initiates execution by receiving a command from NPU to perform a specific collective on a dataset. The command includes the collective type and the memory range address of data residing in the main memory. The messaging agent then divides the dataset into multiple chunks and begins processing \& scheduling of each chunk individually and in a pipelined manner.

The chunk itself decomposes into multiple messages and the collective algorithm runs on the message granularity. As an example, if the chunk has 8 messages and the messaging agent wants to perform an all-reduce in a ring with 4 NPUs, it divides the messages into 2 sets of 4-message size each and executes the sets in serial. In the ring based algorithms, We call such set an \textbfoperations{operation set} because ring-algorithms operate on each set individually. Since in the ring algorithm, different nodes access to different messages within an operation set, this indicates that \textbf{the messages of the same operation set must reside in the same FIFO slot} to ensure that different nodes have access to every messages while performing collective regarding that set. Multiple operation sets can however fit within the same slot.

Each message comprises of one or more packets when it enters the network layer. Each packets is then splitted into multiple flits and each flit consists of multiple phits as it traverses the physical link.
\begin{table}[h]
\caption{Data granularity at different levels of messaging agent execution \TODO{Is this an implementation issue tied to the simulator or is this a design issue. If former we need to move this to the methodology section}}
\resizebox{\linewidth}{!}{\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Granularity}} & \multicolumn{1}{c|}{\textbf{Size}}                                              & \multicolumn{1}{c|}{\textbf{Constraint}}                                    \\ \hline
Set                                    & Training Algorithm                                                              & Training Algorithm                                                          \\ \hline
Chunk                                      & Parameter for Pipelining                                                        & \begin{tabular}[c]{@{}l@{}}Storage Element Size\\ (Area/Power)\end{tabular} \\ \hline
Message                                    & \begin{tabular}[c]{@{}l@{}}Parameter - \\ Multiple Number of Nodes\end{tabular} & Topology                                                                    \\ \hline
Packet                                     & Link Technology                                                                 & Technology                                                                  \\ \hline
Flit                                       & Network Buffer Size                                                                     & \begin{tabular}[c]{@{}l@{}}Microarchitecture\\ (Area/Power)\end{tabular}    \\ \hline
Phit                                       & Link Width                                                                      & Technology                                                                  \\ \hline
\end{tabular}}
\label{tab:garnularity}
\end{table}
\textcolor{red}{some explanation about the contol unit microarch}
\subsection{Walk-Through Examples}
In this section we describe how collectives are performed for hierarchical \& all-to-all topologies. Note that in most parts we use the term message to describe collective operations since this is the unit of data collectives operate on top of. However, every action related to each message means applying that action to all packets within that message since the unit of processing is packet inside the architecture.
\subsubsection{Collectives in the Hierarchical Topology} Figure \ref{fig:hflow_all} shows how the all-reduce operation is done for one chunk of data in the messaging agent for a hierarchical 2D Torus. In this configuration, each FIFO logical partition serves the source for \textbf{only} one phase of the algorithm, thus, there are 4 logical partitions labeled as L1-L4 (excluding DMA FIFOs). In the first phase of of the algorithm (shown in Figure \ref{fig:hflow1}), the chunk data is first transferred into the L1 FIFO (\#1) and then the reduce-scatter operation is done along the local ring (\#2-\#10). The reduce-scatter itself has two different phases. At the first phase of reduce-scatter, the received messages are reduced with the local data (\#2-\#6) and forwarded to the next NPU in the ring using an appropriate output port. \footnote{Note that based on the ring-based algorithm, the very first local message of the operation set is simply forwarded using the EU without any reduction with the received data.}

The second phase is when the last message is received, reduced with the last message, and written back to the logical buffer partition belonging to the next phase of the algorithm (\#7-\#11). In the next phase (Figure \ref{fig:hflow2}), the all-reduce operation is done across one of the vertical rings. The operations (\#1-\#10) perform reduce-scatter and is the same as the previous phase with one exception: during the operation (\#9), the last phase of reduce-scatter is overlapped with the first phase of all-gather and at the same time, the message is both written back to the next phase buffer and forwarded to the next NPU (\#10). This follows by the next steps of the all-gather (\#11-\#12) for that operation set where the received message is again written to the FIFO and forwarded to the next phase. The third phase (Figure \ref{fig:hflow3}) is the same as the second phase with the exception that the all-reduce is now performed across a horizontal link by using L3 as a source buffer.

The last step is the all-gather across a local ring (Figure \ref{fig:hflow4}). The first message is read from the L4 FIFO and is forwarded to the next NPU and the DMA buffer simultaneously (\#1-\#4). The subsequent steps of the current operation set is when a new message arrives. The received message is again  forwarded as well as written to the DMA buffer using the direct link (\#5-\#7). Finally, the data is sent back to the NPU memory (\#8).

\begin{figure*}[h]
  \centering
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/page-2.pdf}
    \caption{step 1 of the hierarchical all-reduce. In this step, the reduce scatter is performed among the tiles within the same package.}
    \label{fig:hflow1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/page-3.pdf}
    \caption{step 2 of the hierarchical all-reduce. In this step, the all-reduce (reduce-scatter+all-gather) is performed among the tiles connected by the vertical inter-package links. The actions 1-10 are the same as 2-11 in step 1.}
    \label{fig:hflow2}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/page-4.pdf}
    \caption{step 3 of the hierarchical all-reduce. In this step, the all-reduce is performed among the tiles connected by the horizontal inter-package links.}
    \label{fig:hflow3}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/page-5.pdf}
    \caption{step 4 of the hierarchical all-reduce. In this step, the all-gather is performed among the tiles within the same package. At the same time, the final data is directed to the output FIFOs and then it is sent back to the main memory.}
    \label{fig:hflow4}
  \end{subfigure}
  \caption{The all-reduce operation exmple for one chunk of data in a hierarchical 2D torus topology.}
  \label{fig:hflow_all}
\end{figure*}
The all-to-all collectives are straightforward. In all steps, the RAMs are the single source and destination entity. The data size does not change during different steps of all-to-all. So, a fixed contiguous space for a chunk is reserved in the RAM. The final step is the movement of the data from RAM into the DMA buffer and deallocating the space of the chunk from the RAM.
\subsubsection{Collectives in the All-to-All Topology}
Figure \ref{fig:af_all} shows how all-reduce for one chunk is done in an all-to-all topology with 3 NPUs that are fully connected using inter-package links. The FIFOs are partitioned into the 3 logical groups labled as L1-L3 (excluding the DMA FIFOs). The number of buffers in the second and third logical group should be at least the number of NPUs participating in the all-to-all topology. The first phase (Figure \ref{fig:af_1}) is like phase 1 of hierarchical topology (Figure \ref{fig:hflow1}) and performs reduce-scatter in the local dimension. But unlike hierarchical topology, the results are scattered across multiple FIFOs.

In the second phase (Figure \ref{fig:af_2}), the data of of 2 buffers (out of 3) are simply forwarded to the other 2 NPUS (inter-package) while at the same time, the data in one of the buffers is written into the buffers of the L3 (\#1-\#4). The received messages are alos written back to L3 group. These accumulated data in L3 should be reduced during the next phase.

Figure \ref{fig:af_3} shows the third phase in which one (or more) EUs iterate over the 3 buffers of L3 and read one packet from each buffer in three subsequent read operations in order to reduce them (\#1-\#3). When one packet is reduced by EU, the EU broadcasts it to other (inter-package) nodes as well as writing it to one of its buffers (\#5-\#6) again in L3. This process continues until all packets residing initially residing in the buffers are reduced. The messaging agent then stores the received messages into their corresponding FIFO (\#7-\#9) in L3. Note that here, the source and destination buffers belong to the same logical group. The reason is that when the third logical group is executing collective, its corresponding second logical group can not proceed because they share the same physical ports. This allows the data to be written to the same group without any contention.

Figure \ref{fig:af_4} shows the last phase of all-reduce that is an all-gather across the local dimension. This is similar to the las phase of hierarchical all-reduce (Figure \ref{fig:hflow4}) with the exception that here, the 3 buffers initiates three different all-gathers but in-serial. The other collectives of the all-to-all topology are straightforward. \textcolor{red}{can be expanded}

\begin{figure*}[h]
  \centering
  \begin{minipage}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/page-6.pdf}
    \caption{step 1 of the all-to-all topology all-reduce. In this step, the reduce scatter is performed among the tiles within the same package and the reduced data is scattered across multiple FIFOs.}
    \label{fig:af_1}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/page-7.pdf}
    \caption{step 2 of the all-to-all topology all-reduce. In this step, the data is forwarded to to the output ports (except the local-data FIFO that is redirected to the next phase FIFO) and at the same time, received data are stored for the next phase.}
    \label{fig:af_2}
  \end{minipage}
  \begin{minipage}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/page-8.pdf}
    \caption{step 3 of the all-to-all topology all-reduce. In this step, the ALU is iterating over FIFOs and fetch one element per FIFO accumulates the results. After one result is ready, it broadcasts data to the output ports as well as writing it back for the next phase.}
    \label{fig:af_3}
  \end{minipage}
  \begin{minipage}[b]{0.49\linewidth}
    \includegraphics[width=\linewidth]{figs/page-9.pdf}
    \caption{step 4 of the all-to-all topology all-reduce. In this step, the all-gather is performed among the tiles within the same package. At the same time, the final data is directed to the output FIFOs and then it is sent back to the main memory.}
    \label{fig:af_4}
  \end{minipage}
  \caption{The all-reduce opeartion exmple for one chunk of data in a an all-to-all topology with 3 NPUs in the fully connected nodes.}
  \label{fig:af_all}
\end{figure*}

\subsection{Data Management Model}
The way data is managed \& moved  inside the messaging agent is to maximize the messaging agent utilization while keeping the control unit logic simple. In our design, data chunks traverse different logical FIFOs during different phases of the collective and they are processed when they are at the head of FIFO. The alternative approach is to allocate a constant space for a chunk and use that space during all phases of the collective. However, this is not efficient way of using valuable on-chip storage due to one important property of collective operations: the data size might change during different phases of the algorithm. Thus, allocating a constant space wastes on-chip storage or requires sophisticated dynamic allocation/de-allocation schemes to manage free spaces, adding complexity to both datapath and control unit. Using logical FIFOs for different phases allows for a fine-grained yet low complexity storage allocation/de-allocation scheme as chunks go through different phases, as well as simplifying the control logic to deal with the simpler FIFO interface compared to the RAMs. Note that in all-to-all collectives, data size remains constant, hence, allocating a reserved storage in RAM does not waste any space.

When using FIFOs, cares must be taken to prevent unintended under-utilization caused by the limitations of the FIFO interface. If there is a pending chunk scheduled on an idle port, the design should not fundamentally restrict the execution simply because data is not reachable inside the logical FIFO. To address this challenge, three questions must be answered: 1-How many FIFOs must be provided? 2-How should they be allocated to the ports? 3-what should be the size of each FIFOs? 

Here, we provide a systemic way of answering to the above questions. 
First, for the collective algorithms where the size of data is always constant (e.g. all-to-all), one logical group of RAMs is sufficient to serve as the source for all phases. For other algorithms without this property, assuming a collective has $N$ phases, we start by creating $N$ logical groups (excluding DMA FIFOs) each serving as a source for one phase. Each phase of the algorithm operates on a number of input/output port pairs. Assume $Port[i]\; (1 \leq i \leq N)$ gives the number of involved ports pairs in $i$'th phase of the algorithm, the the total FIFOs for logical group $i$ should be at least $MAX(Port[i],Port[i-1])$. Also, the FIFOs within the logical group $i$ should be allocated to port pairs of phase $i$  with respect to the port bandwidth (e.g. spread FIFOs equally among all port pairs if they all have the same bandwidth). The term $Port[i]$ ensures that the port pairs within logical group $i$ have always access to one FIFO read port. The second term $Port[i-1]$ guarantees that all ports in phase $i-1$ can proceed the execution of their chunks since they have access to at least one write port of the logical buffers in phase $i$. If two consecutive phases $i$ and $i+1$ work on the same ports, the the logical group $i$ and $i+1$ can be fold to one logical group since phase $i-1$ and $i$ can not proceed at the same time. This is exactly what the case for phase 2 and 3 of the all-reduce in the all-to-all topology. Since these 2 phases use the same ports, the logical group 3 and 4 are fold to one as explained in the walk-through example.

The answer to the 3'rd question however, is dependent to the bandwidth of the ports and the optimized values are determined by the simulation. 
The concept of distributed storage for performing each phase in a separate storage element might introduce the deadlock problem if the storage elements have the cyclic dependency. However, the concept of logical partition for each phase and one-sided flow of data among partitions ensure deadlock freedom.

Finally, it is worth noting that the logical FIFOs are selected as the primary storage element because it is the simplest interface that
addresses all of the data management requirements of the target systems. To provide more compatibility to the future collective algorithms, one can increase the degree of the random accesses by increasing the slot size as described earlier. The extreme to this approach is to replace FIFOs with RAMs. However, the concept of logical buffers per each phases and the flow of data remains constant to provide efficient storage management, port utilization and deadlock-freedom. It is then the responsibility of the designer to trade between the complexity and future compatibility.

\subsection{Software Interface}



==> sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}

\subsection{Message Fusion}
DL frameworks, such as Google's TensorFlow and Facebook's Pytorch, and communication libraries, such as NCCL, support an optimization called \emph{message fusion} that combines multiple gradient communication operations across different layers and issue a single large allreduce. Message fusion helps alleviate the overheads of launching multiple kernels and enabling higher bandwidth utilization given larger messages. However, it is comes at a cost of extra memory copies and does not utilize the available compute-communication overlap. While optimizations such as message fusion are critical in getting the best performance, we believe the key problem is the under-utilization of network bandwidth due to inefficient communication datapath.  

\subsection{Direct cache injection}
Direct cache injection allows the NIC to directly write to the last level cache. This has been supported in Intel Xeon processors under the codename \emph{Data Direct IO}. This allows the NPUs to read remote directly directly from last level cache at potentially higher bandwidth than HBM memory. While this could potentially overcome congestion on the memory bus, it introduces a new set of challenges which needs further investigation. For starters, this could potentially lead to higher capacity misses of critical compute data if communication starts pushing data directly into caches. Further, this introduces additional architectural/micro-architectural complexity. We believe a dis-aggregated design that decouples messaging/network from the compute provides better flexibility to improve the system from one generation to another. 

% \subsection{Shared memory within package}
% We made this design decision for two reasons: first, optimizing for \emph{Non-Uniform Memory Access} (NUMA) and shared memory is challenging - as evident from extensive work on HPC workloads for CPUs. % \cite{}.
% Additionally, having two separate communication paths, i.e. shared memory within package and message passing across packages; increases the scheduling and optimization complexity for various collective algorithms. Therefore, we assume explicit communication between NPUs within a package through a high-performance topology aware communication library. This programming model also allows scaling the number of modules within a package with improvements in packaging technology. While the NIC is depicted as a distinct chiplet, the challenges discussed in this paper are also applicable to when the NIC is physically integrated into the NPU chiplet. This requires supporting a cache-coherent interface for NIC to integrate into the on-chip fabric, increasing design complexity and fundamentally constraining NPU and NIC improvements across product generations. Such design choices are important for future accelerator systems and warrant a separate study. 

%While enabling a shared memory abstraction across NPUs within a package presents a simpler programming model, optimizing for NUMA and shared memory are challenging - as evident from extensive work on HPC workloads for CPUs. Therefore, we propose explicit communication between NPUs within a package through a high-performance topology aware communication library. 

%\subsection{Compression and Sparse Collectives}


==> sections/extra_figs.tex <==
%\insertWideFigure{overview}{TODO}
\begin{figure*}[!t]
  \centering
  \begin{subfigure}[b]{0.9\linewidth}
    \includegraphics[width=\linewidth]{figs/Architecture2.pdf}
    \caption{Overview of Baseline vs. Proposed System. NPU = Neural Processing Unit (e.g., GPU/TPU)}
    \label{p1}
  \end{subfigure}
  \begin{subfigure}[b]{0.9\linewidth}
    \includegraphics[width=\linewidth]{figs/NewCommunicationFlow1.pdf}
    \caption{Collective Communication Timeline during Distributed Training in Baseline.}
    \label{p2}
  \end{subfigure}
  \begin{subfigure}[b]{0.9\linewidth}
    \includegraphics[width=\linewidth]{figs/NewCommunicationFlow2.pdf}
    \caption{Collective Communication Timeline with Proposed Messaging Agent.\TODO{@Saeed - remove word Cocoa from figure and change it to NCU}}
    \label{p2}
  \end{subfigure}
  \caption{Motivation: \todo{Need caption}}
\label{fig:motivation}
\end{figure*}


==> sections/introduction-bkp.tex <==
\section{Introduction}\label{sec:intro}

\TODO{Rewrite - identify the challenges in baseline systems today. And say that it becomes worse in future systems. Move Fig 3 as Fig 1}

% Overview:  
%- DL workload demands are increasing
%- DL compute accelerators are adding a lot of compute
%- There is no work on (a) topology and (b) how to build efficient endpoint to drive that topology
%- This work assumes two topologies: switch based partial alltoall and torus both with high BW local dimension
%- Given this... we provide the motivation in terms of challenges in driving the network and design for new messaging agent. Emphasize the following: why endpoint design is critical and motivation for our work. Challenges w/ endpoints - memory contention, cores for compute, etc. 


Deep Learning (DL) and Deep Neural network (DNN) models are being deployed pervasively across a wide range of real-world application domains such as image classification, natural language processing, and autonomous driving. The size and computational requirements of these DNN models are growing at an unparalleled rate, 2x every 3.4 months \cite{OPENAI}, to handle the unrelenting growth in data and workload requirements. %A recent study by OpenAI showed the growth in DNN model sizes of 100000x in 18 months (compared to historical growth of Moore's law at 2x every 18 months) \cite{}. 
The advent of energy-efficient inference accelerators capable of handling these large models and need for accelerating training time when dealing with 10s to 100s of petabytes of input data is raising the demand for faster and more efficient DL training solutions. This can only be achieved through scalable and efficient distributed training, since a single accelerator cannot satisfy the compute, memory, and I/O requirements of today's state-of-the-art DNNs. 
%Scaling DL training workloads, especially synchronous \emph{Stochastic Gradient Descent} (SGD), is a challenging problem on today's platforms and will only get harder in future training platforms, and is the focus of this work.

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.45]{figs/compare.pdf}
\end{center}
\caption{Baseline system vs. ACE}
\label{fig:baselinsVsACE}
\end{figure}

%\begin{figure}[t]
%\begin{center}
%\includegraphics[scale=0.35]{figs/architecture4.pdf}
%\end{center}
%\caption{Asymmetric Hierarchical Scale-up Accelerator Design}
%\label{fig:architecture}
%\end{figure}

\insertWideFigure{collectives_table}{Overview of collective communication operations used in DNN training networks.}

Today's DL Training platforms are built by interconnecting multiple accelerators, henceforth called \emph{Neural Processing Units} (NPUs), together through different network fabrics, running distributed DL training algorithms. Distributed DL training is highly communication intensive, with collective communication operations (such as all-to-all and all-reduce) used to synchronize input/output/error activations during the forward/backward pass, and gradients during the backward pass,
depending on the parallelization strategy (data/model/hybrid) employed. There has thus been extensive work on optimizing DL training communication on current platforms; spanning algorithms \cite{DBLP:journals/corr/KeskarMNST16,DBLP:journals/corr/GoyalDGNWKTJH17}, frameworks \cite{intelcaffe,tensorflow,ngraph}, communication libraries \cite{mlsl,DBLP:journals/corr/abs-1708-02188,nccl}, and high-bandwidth interconnects~\cite{NVlink}.

Parallelization is often done through hierarchy of NPU networks: (i) scale-up and (ii) scale-out networks.\emph {Scale-up} networks connect accelerators within/across one or more chassis/rack directly, through high-bandwidth interconnect fabric, and do not require CPU host involvement in the communication data-path~\footnote{In contrast the \emph{scale-out network}, i.e. the network connecting host CPUs together through Ethernet, require accelerators to rely on the host for both control/datapath. Hence, scale-out is used to connect individual scale-up networks. This will be explored as part of future work.}. However, there is \textit{limited or no work in systematically addressing system and architectural bottlenecks that inhibit efficient network bandwidth utilization in current/future training platforms in the \textbf{scale-up} level - the focus of this paper.}

Figure \ref{fig:baselinsVsACE} shows the NPU architecture and its connected peripherals. As the figure shows for the baseline system, handling collective communication on NPU cores have three major overheads: (i) it consumes valuable NPU compute resource for driving the network and performing collective algorithm, rather than performing actual training computation (compute overhead), (ii) it congests both \emph{NIC-NPU} and \emph{MEM-NPU} busses, resulting in more latency to handle communication (communication overhead), (iii) and it reduces the MEM bandwidth available for actual training computation (compute overhead). 

Figure \ref{fig:baselinsVsACE} also shows our proposal, \emph{Accelerator Collectives Engine (ACE)}, that is designed to mitigate such effects by offloading the communication to a customized NIC designed to handle distributed DL training collective patterns and cope with the high bandwidth demand of scale-up network. This way: (i) NPU resources are totally free to perform training algorithms only, (ii) The MEM-NPU and NIC-NPU busses are significantly less congested and are used only for initial/final data-transfer to/from ACE on-chip memory, (iii) there are much more memory bandwidth available for training computation.      

Then, we describe the architecture of ACE, a novel offload accelerator for DL collectives. Unlike prior work in SmartNICs for CPUs \cite{NIC1,NIC2}, our communication offload solution is designed for scale-up topologies with orders of magnitude higher BWs than traditional flat scale-out networks. 

Finally, we quantify the benefits of the proposed design using micro-benchmarks and popular DL models, such as ResNet-50a and Transformer \cite{Transformer}, using an end-to-end DL training simulator~\cite{traccsim}. Our end-to-end methodology enables evaluating various design choices across DNN model, DNN parallelism and corresponding communication patterns, framework-level optimizations, design/mapping hierarchical collective algorithms, endpoint design, fabric design, fabric topology, and finally the interactions between these individual components. Given the large design space, we present results comparing our proposed communication accelerator against a baseline solution (where NPU cores are driving both compute and communication operations) for collectives-based synchronous training on 2D-Torus (inspired by Google's TPU platform \cite{TPU}) and fully connected switch-based topology (inspired by NVIDIA's DGX-2 platform \cite{dgx2}).
To summarize, this paper makes the following novel contributions:
\begin{itemize}
    \item Establish the challenges in scaling DL training workloads, esp. as related to accelerator systems for scale-up networks. 
    \item Propose a novel offload engine, called \emph{Accelerator Collectives Engine} (ACE), designed to work efficiently in the scale-up network and tuned to handle collective communication. 
    \item Present an end-to-end methodology for modeling the training loop for different parallelism models and modeling both compute and communication time.
    \item Finally, demonstrate ACE achieves \todo{XX}$\times$ speedup for modern DL workloads such as ResNet50 and Transformer over a state-of-the-art bandwidth-equivalent baseline.
\end{itemize}

The rest of the paper is organized as follows: \autoref{sec:motivation} establishes the challenges in scaling DL training, specifically focused on critical bottlenecks in the endpoint that inhibit efficient NW utilization. \autoref{sec:design} describes our novel micro-architecture, called \emph{Accelerator Collectives Engine} (\ncu), for accelerating hierarchical scale-up traffic. This is followed by a detailed description of our evaluation and simulation methodology in \autoref{sec:methodology} and the experimental results in \autoref{sec:results}. Next we compare our work against related work in \autoref{sec:related}. We conclude the paper by briefly describing our next steps in \autoref{sec:conclusions}.


==> sections/offload.tex <==

When it comes to the previously proposed communication offload schemes, they can be categorized into two groups: i) switch-based offload methods (e.g. NVIDIA's switch offload \cite{InNetwork}), and ii) endpoint-based methods such as \ncu. \autoref{tab:SwitchVsEndpoint} shows the comparison between these two. Both methods reduce the burden on endpoint memory and compute for handling communication related tasks. However, endpoint-based based methods are more flexible in supporting various network topologies, as opposite to switch-based methods that require switch in the network topology and hence, point-to-point (PTP) links do not benefit from the offload scheme. Note that in scale-up domain, many platforms are designed solely using point-to-point network topologies (e.g. NVIDIA DGX-1 \cite{DGX1} and Google TPU \cite{TPU}). This is in addition to the intra-package networks that are almost always PTP  \cite{SiliconInterposer}. Additionally, unlike switch-based methods that only support a single reduction/broadcast traffic pattern to/from the switches, endpoint-based methods can support many different algorithms (patterns) (e.g. ring, halve-doubling, double-binary-tree, etc.). The above reasons show why endpoint-based methods such as \ncu is a better investment for the scale-up network.


Another point of difference between \ncu and previous offload based schemes  \cite{NIC1,NIC2,SHARPProtocol,CommBottleneck1,CommBottleneck2,IncBricks,NetCache} is that almost all of them focus on scale-out domain and require CPU intervention.   
However, these CPU-initiated schemes require explicit resource reservations that will be exacerbated for scale-up network that has large number of network packets, eventually limiting the scalability. We contrast \ncu against prior works on switch/endpoint-offload in  \autoref{table:related_offload} (visualized in \autoref{fig:overviewOfServer}) and discuss differences in \autoref{sec:related}. To summarize: \textbf{\textit{This is the first endpoint-based offload scheme that is tuned for distributed training in scale-up networks.}}


==> sections/outline.tex <==
\section*{Outline}

\textbf{What is Terminology?}

\textbf{GPUs today use SMs to perform the messaging agent tasks.}

\textbf{Shared Address Space.}

\textbf{Paper Outline:}
\begin{itemize}
\item \textbf{Intro:} 
\item \textbf{Background:}

1.Distribution Training.

2.Compute + Communication 
\item \textbf{Compute:}
1.GEMM, Gradients etc etc [cite]
\item \textbf{Communication (Put as a Table):}

1.Orchestrator (Today - CPU/SM. Proposed: Messaging Agent).

2.Packet Processor (Today - CPU/SM. Proposed: Messaging Agent).

3.Marshalling / Demarshalling (Today - NIC. Proposed: Messaging Agent).

4.Network Traversal (Today - Off-chip. Proposed: Off-chip + On-package).

\item \textbf{Motivation:}
\item \textbf{Evolution of Workloads (Compute and Memory Characteristics):}

1.Model sizes have improved 100K  times over 2-3 years: openAI chart.

2.Data Parallel vs Model Parallel.

3.Today -- Data Parallel.

4.Future -- Model Parallel, Hybrid Parallelism, embedded tables.
\item \textbf{Compute Nodes:}

1.Compute is becoming efficient - sparsity, lower precision.

2.Will not fit within one tile due to compute area and memory sizes  and limited BW => Need Scalability.
\item \textbf{How to Scale?:}

1.Scale-out (Across Boards - Today).

2.Scale-up (Adding Tiles on-package and also on board).
\item \textbf{Bottlenecks / Challenges at End-Points Today:}

\item \textbf{Qualitative:}

1.Bandwidth: 1.How to provide raw BW => HBM, 2.How to drive this BW.

2.Compute Utilization
\item \textbf{Quantitative:}

Real system (CPU/GPU).

Ideal Baseline (using Garnet - Same params as Real-System, and sweep Mem BW and Compute Utilization params)
\item \textbf{Contributions of this paper:}

1.Highlight Challenges and Bottlenecks (via real-system and simulator): Both at multi-tile.

2.Proposal: Messaging Agent: 1.Hardware, 2.Topology etc.

3.Co-Design of the Orchestration + Messaging Agent

4.Performance improvement by XXX 
\end{itemize}

\TK{Two TODOs: (i) Baseline Pipeline (for both paper 1 and 2, (ii) innovation pipeline to decide messaging agent microarch}

Terms: NIC (host-side) -> HFI -> Messaging Agent (functionality - could be software thread on CPU/GPU or HW engine)

CPU/GPU/smartNIC - common names.

Functionality: Messaging Agent.
Proper Name of Proposed Accelerator.

\section*{TODOs}

Figures:
\begin{itemize}
    \item High-level figure showing DL training over scale-up system.
    \item Baseline and Proposed Systems with NIC Microarch expanded [IN PROGRESS]
    \item \TK{In NIC Microarch: show 3 flows: (a) Dense All Reduce, (b) Decompress + Dense All Reduce + Compress (c) Sparse All Reduce}
    \item Communication Flow [DONE]
    \item Table showing communication behavior in different DL models.
\end{itemize}


Simulator Status + TODOs:
\begin{itemize}
    \item Hierarchical Collective -> Yes: ring, torii, glueless, NVswitch, all-to-all. We can also do flat all-reduce.
    \item Compression => sparse collectives -> No. Need to decide compression algo, HW for it, sparse reduction etc.
    \item Microarch of MA Engine for collective offload and scheduling, sparse computations, ... -> No: (i) Need a block diagram (use triggered instructions as reference picture) (ii) Extend Garnet appropriately on the compute side, (iii) RTL for building blocks
    \item Message Sizes: For Dense - size always same, for Compression - size depends on compression algo and data, for Sparse Collective - delay depends on data. How to handle compression and sparsity?
    \item Integration of MA Engine within the DL Training Pipeline -> Yes/No.
    \item Mechanism for deciding degree of offload on to MA Engine -> No (Need to model baseline in more detail)
\end{itemize}

Writing - Srinivas and Sudarshan





==> sections/related_old.tex <==
\section{Related Work}\label{sec:related}
\vspace{-2mm}
%\TODO{contrast against switch offload - barefoot networks and NVIDIA ISCA 2020 paper. we support any topology, they rely on switch-based}

%{\TK{@Saeed: Pls add table qualitatively comparing against SPIN: Target Workloads, Programming Model, Offload Model, Hardware}}
\begin{comment}
We broadly classify related work into three categories: (i) optimizing communication through software (ii) accelerator fabric and scaling exploration and (iii) scale-out smart NICs and collective offload on switches. 

\textbf{Optimizing Communication in DL platforms}
Two classes of solutions exist today to to optimize communication within DL training platforms.
The first, is to \textit{reduce the amount of communication}.
These solutions fall within the realm of optimized communication algorithms~\cite{DBLP:journals/corr/KeskarMNST16,DBLP:journals/corr/GoyalDGNWKTJH17} and 
parallelism strategies~\cite{zero,nccl, mlsl}. While most training workloads 
leverage data-parallelism for this reason (as it involves 
lesser communication), in many cases model/hybrid parallelism is inevitable due to the size of the model~\cite{dlrm, zero}. Moreover, collective communication inherently requires communicating updates proportional to the size of the model making it hard to reduce the amount of data to be communicated.
The second class of solutions fall within the realm of 
\textit{overlapping communication with compute}.
Topology-aware collective algorithms from DL libraries like Intel's MLSL~\cite{mlsl} and NVIDIA's NCCL~\cite{nccl} target such an overlap, and are preferred over running collective algorithms via MPI like HPC systems. However, as we showed in this work, getting a perfect overlap is 
challenging due to contention for compute and memory at the endpoint.


\textbf{Accelerator Fabric and Scaling.}
In terms of collective algorithms, many works suggested and examined different algorithms based on different assumptions. Thakur et al. \cite{collective1}  analyzed algorithms based on the constant overhead between each two communicating node. Authors in \cite{collective2} extended the collective operations for nodes with the ability to send/multiple messages. Patarasuk et al. \cite{collective3} introduced a bandwidth efficient all-reduce for clusters of workstations. However, these algorithms mainly targeted the scale-out network or they analyzed the algorithms using simplified assumptions for the systems that are not realistic in the actual systems. 
Circuit level techniques to enhance the memory bandwidth for deep learning training/inference workloads have also been explored~\cite{mcm-gpu,DLCircuit}.
\end{comment}

%Arunkumar \textit{et al.}~\cite{energy_efficiency_mcm} proposed an energy cost model for multi-chip scaleup design. An energy-cost model could be integrated to our work and we leave this as future work.

%\subsection{DL communication accelerator via compression}
%Authors in
%\cite{DLCompression,DLCompression2,Scale_out_training,Hadi1} proposed compression for training %algorithms to reduce the communication size. The authors in \cite{inception} propose %compression hardware features in the NIC for reducing volume of communication gradient. %Compression features could be added to our smart messaging agent which we leave it to future %work.
%The other work in \cite{cDMA} proposed compression inside the DMA engine to boost the data %transfers between CPU memory and GPU memory for training workloads. Kwon et al. %\cite{beyondMemoryWall} adresses the host (CPU) to device (accelerator) memory communication %wall by moving the memory modules to the device side interconnect. Authors in %\cite{distributed_learning} analytically modeled the cost of different parallelism schemes for %a given network dimension in terms of communication size between the nodes, and suggested the %best parallelism decision to employ for each network. These methods are orthogonal with \ncu %and can be used in parallel.

%\subsection{Scale-out SmartNICs and Collective Offload on Switches}

%\textbf{Scale-out SmartNICs and Collective Offload on Switches}
%Communication offload is not a new idea.

%Over the years, many schemes have been proposed to improve the communication performance for ML, HPC, and  general-purpose computing by leveraging offload on NICs and switches. Our work differs from prior efforts in that we focus on SmartNIC-based collectives for DL training. 

%The key difference between all prior works versus ours is that their is \textit{scale-out}, while \ncu focuses on \textit{scale-up}. As explained in \autoref{sec:intro}, these CPU-initiated schemes fail to scale properly and are extensive in terms of resource usage for the scale-up network. 

\ncu is the first work proposing a dedicated hardware engine at the endpoint for running DL collectives within the Accelerator Fabric.
The works closest in flavor to \ncu 
are those on 
%Previous work have demonstrated the efficiency of 
collective offload to either smart NICs or network switches 
for datacenter networks. We contrast them in \autoref{table:related_offload} and discuss them here.
These works can augment \ncu when
scaling training 
to beyond one training platform (\autoref{fig:overviewOfServer}) and ripe for future work.
% , ACE is an AFI extension for accelerator-based systems and can be integrated in different system topologies such as switch based or point-to-point (e.g. Torus) systems.

\textbf{Communication offload to SmartNICs.}
%The concept of designing a NIC and protocol pair for offloading the network tasks in the scale-out network are proposed in \cite{NIC1,NIC2}. More specifically,
Prior SmartNIC solutions for collective offload, such as \cite{NIC1,NIC2}, focused on scale-out datacenter networks and HPC workloads. Triggered collectives \cite{NIC1} is the closest comparison to ACE but is specific to Portals transport and CPU-based scale-out systems while ACE is transport-agnostic and sufficiently flexible to support hierarchical topologies (local + scale-up). Unlike both Triggered collectives \cite{NIC1} and ACE, sPIN \cite{NIC2} uses ARM cores and will not be able to drive high bandwidths required for DL platforms. 
%
INCEPTIONN \cite{Hadi1} proposes a Smart-NIC based compression offload for parameter servers for DL training. The inherent differences between parameter server vs. collectives makes ACE vs. INCEPTIONN comparison out of scope for this paper. 
%
HPC systems with Torus-based topology, such as BlueGene \cite{BlueGene}, PERCS \cite{PERCS}, and Anton2 \cite{Anton}, have supported collective offload on network routers. SmartNICs are more flexible than routers found in such system since routers are purpose-built for the target topology. 

Numerous other proposals have demonstrated the benefits of SmartNICs for communication offload but do not address the requirements of DL training. Microsoft's Brainwave \cite{Brainwave} proposes a bump-in-the-wire SmartNIC for distributed inference. IncBrinks \cite{IncBricks} proposes distributed in-network caches on the scale-out network, which store key-value pairs for frequently accessed data. They allow simple operations such as increment to be done using a simple in-network processor. NetCache \cite{NetCache} uses the ASIC within a switch to do dynamic caching and load-balancing of requests to that switch. 

%The authors in \cite{NIC1} proposed designing a triggered based architecture that will trigger collective communications based on listening to the certain network events defined by the programmer. sPIN NIC (proposed in \cite{NIC2}) allows the programmer to offload packet handlers that processes different types of packets upon arrival using available compute resources inside the NIC. \textcolor{red}{Some proposals used FPGAs as smart NICs for inference \cite{Brainwave} or training \cite{Hadi1}. However, compared to \ncu, these approaches (i) are not designed for handling various collective communication algorithms, (ii) are proposed for loosely coupled network of accelerators with much less network bandwidth and higher latency requirements, and (iii) require a FPGA resource and that is more costly.}

\textbf{Communication offload to Switches}
Switch-based offload solutions, such Intel's Barefoot \cite{Barefoot}, Mellanox SHARP~\cite{Mellanox}, and NVIDIA's shared memory switch offload \cite{InNetwork}, have proposed aggregation in switches. In contrast to SmartNIC-based collective offload solutions, Switch-based solutions have two major disadvantages: (1) they are inherently limited to switch topologies while SmartNICs are more flexible and support point-to-point (e.g. Torus) and switch topology, (2) they have higher constraints on compute and memory resources given the large number of endpoints connecting to the switch. SmartNIC based solutions overcome this by distributing the resource requirement across endpoints. More specifically, Barefoot \cite{Barefoot} offload scheme requires operating on quantized integer values (due to lack of floating point arithmetic in the switch) potentially affecting training accuracy for future DL models. On the other hand, NVIDIA's switch-based offload \cite{InNetwork} is purpose-built for shared memory allreduce collectives; limiting the number of endpoints and types of collectives that can be supported. Switch offload has also been explored for accelerating Reinforcement learning~\cite{CommBottleneck1}.




%speed up training time by reducing the amount of data transmitted by supporting aggregation in the switches. Collective offload in switches are however limited by on-chip memory the switches can support. Moreover, the  computing units are limited to integer units while DL training requires floating point. Authors in \cite{CommBottleneck1} proposed adding an accelerator per switch to implement in-switch reduction. 

%\TODO{need text for switch vs end points}

%\TODO{need some points about having more flexibility as we can support arbitrary algorithms, topologies. Switch has to handle data from multiple end points so limited by buffering etc. Fixing at end point distributes the resource requirement instead of aggregating it at the switch which has limited buffers...}

%\TODO{@Sudarshan -- some lines about the fact that switch-based offload will be constrained by what the switch can do.}

%\textcolor{red}{Recently, the switch-based offload scheme is proposed for the scale-up network of GPUs \cite{InNetwork}}. \TODO{only works for all-reduce} Unfortunately, switch-offload solutions only work for switch-based topologies, while \ncu can work for both switch-based and pt-to-pt (like Torus).



%\textbf{Offload on Switches for HPC Collectives.}


%The support for switch-based support is implemented in modern HPC systems like Intel's BlueGene \cite{BlueGene}, PERCS \cite{PERCS}, and Anton2 \cite{Anton}. \textcolor{red}{TODO @Srinivas: need some lines about collectives in HPC applications}.

%\textit{scale-up} and supports various DL collective algorithms and topologies.

%\input{tables/related_offload}

==> tables/mlsl.tex <==
\begin{table}[!t]
\caption{ResNet-50 communication time and NW utilization}
\begin{center}
\begin{tabular}{||c|c|c|c|c|c||}
\hline
\hline
Number cores & 1 & 2 & 4 & 8 & 16 \\
\hline
Time (ms) & 89.8 & 45.1 & 22.2 & 18.4 & 18.0 \\
Utilization (\%) & 17\% & 34\% & 70\% & 84\% & 86\% \\
\hline
\hline
\end{tabular}
\label{tab:mlsl}
\end{center}
\end{table}

==> tables/parallelism.tex <==
\begin{table}
\caption{\small Communication payloads for different parallelism approaches. FP:Forward Pass. BP: Back Pass}
\resizebox{\linewidth}{!}{\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Parallelism} & \textbf{Activations (FP)} & \textbf{Weight grad (BP)} & \textbf{Input grad (BP)} \\ \hline
\textbf{Data} & & \checkmark & \\ \hline
\textbf{Model} & \checkmark & & \checkmark \\ \hline
\textbf{Hybrid} & partially & partially & partially \\ \hline
\end{tabular}}
\label{tab:parallelism}
\end{table}

==> tables/system_parameters-old.tex <==
\begin{table}[htbp]
\caption{System parameters}
\label{tab:SystemParameters}
\begin{center}
\footnotesize
\begin{tabular}{|c|c|}
\hline
\textbf{Parameter} & \textbf{Values} \\
\hline
%\multicolumn{2}{|c|}{\textbf{Communication Mechanisms and Scheduling}} %\\
%\hline
%collectives & All-reduce, All-to-all  \\
%\hline  
%Scheduling & LIFO \\
%\hline
%Algorithm & Enhanced \\
%\hline
%Packet-routing & Software \\
%\hline
\multicolumn{2}{|c|}{\textbf{Intra-Package}} \\
\hline
%--local-packet-size=256 \
Packet size & 256 Bytes \\
\hline
%--tile-link-width=682 \
Per link BW & 200 GB/s \\
\hline
%--local-parallel-reduce=2 \
Link latency & 90 cycles \\
\hline
%--local-rings=2 \ (unidirectional)
\# of links/NPU & 2 \\
\hline
%--local-link-efficiency=0.94 \
Link efficiency & 94\% \\      
\hline
\multicolumn{2}{|c|}{\textbf{Inter-Package}} \\
\hline
%--package-packet-size=256 \
Packet size & 256 bytes\\
\hline
%--package-link-width=136 \
Per link BW & 25 GB/s \\ 
\hline
%--vertical-parallel-reduce=2 \
%--horizontal-parallel-reduce=2 \
%--router-latency=1 \
%--package-link-latency=5 \ (inter-package link, not sure the exact value)
Link latency & 200 cycles \\
\hline
%--vertical-rings=2 \ (bi-unidirectional)
%--horizontal-rings=2 \ (bi-unidirectional)
\# of links/NPU & 4 (bi-directional) \\
\hline
%--package-link-efficiency=0.94 \
Link efficiency & 94\% \\      
\hline
\multicolumn{2}{|c|}{\textbf{NPU and NIC parameters}} \\
\hline
Compute Accel. & 256x256 TPU-like\\
\hline
NPU-NIC BW & 500 GB/s \\
\hline
NPU-MEM BW & 900 GB/s \\
\hline
%--vcs-per-vnet=5 \
%--message-size=1024 \ (variable for baseline since baseline works better if message size grows in proportion to the actual  dataset)
\ncu Message size & 8KB \\
\hline
%--chunk-size=8KB \ (variable for baseline since baseline works better if chunk size grows in proportion to the actual  dataset)
%preferred chunk number & 16 \\
%\hline
%--buffers-per-ctrl-vc=5000 \
\hline
\end{tabular}
\label{tab:system_parameters}
\end{center}
\end{table}

==> tables/topology_details.tex <==

%\begin{table}[h]
%\caption{Topology details}
%\label{tab:TopologyDetails}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{|l|l|l|l|}
%\hline
%Topology &
%  \begin{tabular}[c]{@{}l@{}}Dimension\\ %Notation\end{tabular} &
%  \begin{tabular}[c]{@{}l@{}}Collective\\ %Algorithm\end{tabular} &
%  BW/Dimension \\ \hline
%D torus &
%  \begin{tabular}[c]{@{}l@{}}\textbf{L x V x H} \\ (L is the %\# of\\ NPUs within \\ a package, V\\ is the \#of\\ %inter-package\\ rows, H is the\#\\ of inter-package\\ %columns)\end{tabular} &
%  \begin{tabular}[c]{@{}l@{}}\textbf{Hierarchical}\\ %\textbf{all-reduce:}\\ 1. Ring-based \\ reduce-scatter\\ in %L\\ 2. Ring-based\\ all-reduce in V\\ 3. Ring-based \\ %all-reduce in H\\ 4. Ring-based \\ all-gather in L\\ \\ %\textbf{Hierarchical}\\ \textbf{all-to-all:}\\ 1. Ring-based %\\ all-to-all in L\\ 2. Ring-based \\ all-to-all in V\\ 3. %Ring-based\\  all-to-all in H\end{tabular} &
%  \begin{tabular}[c]{@{}l@{}}1 bi-directionl ring in L\\ %(using 2 intra-packag\\ links/NPU),\\ 1 bi-directionl ring %in V\\ (using 2 inter-packag\\ links/NPU),\\ 1 %bi-directional ring in H\\ (using 2 inter-package\\ %links/NPU)\\ \\ NOTE: If V/L=1, then\\ L/V has 2 %bi-directional\\  rings.\end{tabular} \\ \hline
%Alltoall &
%  \begin{tabular}[c]{@{}l@{}}\textbf{L x P}\\ (L is the \#\\ %of NPUs within\\ a package, P is\\ the \# of %packages)\end{tabular} &
%  \begin{tabular}[c]{@{}l@{}}\textbf{Hierarchical}\\ %\textbf{all-reduce:}\\ 1. Ring-based\\ reduce-scatter\\ in %L\\ 2. Direct\\ all-reduce in P\\ 3. Ring-based\\ all-gather %in L\\ \\ \textbf{Hierarchical}\\ \textbf{all-to-all:}\\ 1. %Ring-based\\ all-to-all in L\\ 2. Direct \\ all-to-all in %P\end{tabular} &
%  \begin{tabular}[c]{@{}l@{}}1 bidirectional ring in L\\ %(using 2 intra-package\\ links/NPU ),\\ 4 fully connected \\ %switches (using\\ 4 inter-package\\ links/NPU )\end{tabular} %\\ \hline
%\end{tabular}
%%\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\caption{Topology details}
\label{tab:TopologyDetails}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Topology/\\ Dimension\\ Notation\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Collective\\ Algorithm\end{tabular} &
  BW/Dimension \\ \hline
\begin{tabular}[c]{@{}l@{}}3D torus /\\ L x V x H \\ (L is the \# of\\ NPUs within \\ a package, V\\ is the \#of\\ inter-package\\ rows, H is the\#\\ of inter-package\\ columns)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Hierarchical all-reduce:\\ 1. Ring-based reduce-scatter in L\\ 2. Ring-based all-reduce in V\\ 3. Ring-based all-reduce in H\\ 4. Ring-based all-gather in L\\ \\ Hierarchical all-to-all:\\ 1. Ring-based all-to-all in L\\ 2. Ring-based all-to-all in V\\ 3. Ring-based all-to-all in H\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}1 bi-directionl ring in L\\ (using 2 intra-packag\\ links/NPU),\\ 1 bi-directionl ring in V\\ (using 2 inter-packag\\ links/NPU),\\ 1 bi-directional ring in H\\ (using 2 inter-package\\ links/NPU)\\ \textbf{NOTE: If V/L=1, then}\\ \textbf{L/V has 2 bi-directional}\\  \textbf{rings.}\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Alltoall/\\ L x P\\ (L is the \#\\ of NPUs within\\ a package, P is\\ the \# of packages)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Hierarchical all-reduce:\\ 1. Ring-based reduce-scatter in L\\ 2. Direct all-reduce in P\\ 3. Ring-based all-gather in L\\ \\ Hierarchical all-to-all:\\ 1. Ring-based all-to-all in L\\ 2. Direct all-to-all in P\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}1 bidirectional ring in L\\ (using 2 intra-package\\ links/NPU ),\\ 4 fully connected \\ switches (using\\ 4 inter-package\\ links/NPU )\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}

==> tables/topology_details_torus.tex <==
\begin{table}[h]
\caption{Topology-aware Collective Details}
\label{tab:TopologyDetails}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}\textbf{Topology/}\\ \textbf{Dimension}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\textbf{Collective}\\ \textbf{Algorithm}\end{tabular} &
  \textbf{BW/Dimension} \\ \hline
\begin{tabular}[c]{@{}l@{}}3D torus /\\ L x V x H \\ (L is the \# of\\ NPUs within \\ a package, V\\ is the \#of\\ inter-package\\ rows, H is the\#\\ of inter-package\\ columns)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Hierarchical all-reduce:\\ 1. Ring-based reduce-scatter in L\\ 2. Ring-based all-reduce in V\\ 3. Ring-based all-reduce in H\\ 4. Ring-based all-gather in L\\ \\ Hierarchical all-to-all:\\ 1. Ring-based all-to-all in L\\ 2. Ring-based all-to-all in V\\ 3. Ring-based all-to-all in H\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}1 bi-directionl ring in L\\ (using 2 intra-packag\\ links/NPU),\\ 1 bi-directionl ring in V\\ (using 2 inter-packag\\ links/NPU),\\ 1 bi-directional ring in H\\ (using 2 inter-package\\ links/NPU)\\ \textbf{NOTE: If V/L=1, then}\\ \textbf{L/V has 2 bi-directional}\\  \textbf{rings.}\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}
